MaxUp: A Simple Way to Improve Generalization of Neural Network Training

We propose \emph{MaxUp}, an embarrassingly simple, highly effective technique for improving the generalization performance of machine learning models, especially deep neural networks. The idea is to generate a set of augmented data with some random perturbations or transforms and minimize the maximum, or worst case loss over the augmented data. By doing so, we implicitly introduce a smoothness or robustness regularization against the random perturbations, and hence improve the generation performance. For example, in the case of Gaussian perturbation, \emph{MaxUp} is asymptotically equivalent to using the gradient norm of the loss as a penalty to encourage smoothness. We test \emph{MaxUp} on a range of tasks, including image classification, language modeling, and adversarial certification, on which \emph{MaxUp} consistently outperforms the existing best baseline methods, without introducing substantial computational overhead. In particular, we improve ImageNet classification from the state-of-the-art top-1 accuracy $85.5\%$ without extra data to $85.8\%$. Code will be released soon.

==> tex/mao_analysis.tex <==
We consider the following empirical quantile surrogate loss:
\[
\E_{\Dn}\E_{\xxi_{[q]}}\max_{\xxi_{i},i\in[q]}\ell(\x+\xxi_{i},y;f_{\th}),
\]
where $\xxi_{i}$ are i.i.d. sample drawn from some distribution.
We learn the parameter $\th$ by minimizing the above surrogate loss.

\section{Conceptual Examples}
In this section, we want to show how MaxUp can benefit the generalization, with some simple conceptual examples. 
% \section{How Does It Benefits the Learning?}

% A key problem we want to address is that how this method benefits the
% learning. 
\subsection{Linear Binary Classification}

We denote $\mathcal{Y}=\{-1,+1\}$ and let the hypothesis set $\F\in\R^{\mathcal{X}}$
be a set of linear functions for $\x\in\mathcal{X}$. To be specific,
we define $f_{\th}(\x)=\th^{\top}\x$ and set $\F=\{f_{\th}:\left\Vert \th\right\Vert \le R\}$.
The label is predicted by the sign of $f_{\th}(\x)$. We assume the
loss function is
\[
\ell(f_{\th}(\x),y)=\varphi(y\th^{\top}\x),
\]
where $\varphi:\mathbb{R}\to[0,B]$ is monotonically non-increasing
and $L_{\varphi}$-Lipschitz, e.g. the Hinge Loss. 

We consider the Gaussian data augmentation, i.e. $\mathbb{P}(\cdot|\x) = \x + \xxi$ where $\xxi\sim\mathcal{N}(0, \sigma_{\xxi}^2 \boldsymbol{I})$. 
% We want to compare the generalization of the vanilla ERM, ERM with data augmentation and MaxUp.
The function class of MaxUp for this case is:
% We define the following function class for ERM with data augmentation and MaxUp respectively:
\begin{align*}
    % \hat{\mathcal{F}} = & \left\{f_{\th}(\x):=\mathbb{E}_{\xxi}\th^{\top}\left(\x+\xxi\right)y:\left\Vert \th\right\Vert \le R\right\}, \\
    \tF= & \left\{ f_{\th}(\x):=\E_{\xxi_{[q]}}\min_{\xxi_{i},i\in[q]}\th^{\top}\left(\x+\xxi_{i}\right)y:\left\Vert \th\right\Vert \le R\right\}.
\end{align*}

% {\color{red} [TR: Feel the notation is a little confusing, maybe use $\mathbb{E}_{\xi_{[q]}\sim \mathcal{N}(0, \sigma_\xi^2 I)}$?]}

% And similarly, we have $\Rn[\ell \circ \tF]\le L_{\varphi}\Rn[\tF]$. 
Here we show that, {\color{red} under some mild assumption}, our method can improve the generalization on the clean data.


\begin{theorem}[Gaussian Adversarial Rademacher Complexity]
\label{thm:weak}
We have that
\begin{align*}
    \Rn[\tF]\le\Rn[\F]+\frac{G_{q,R}}{2\sqrt{n}},
\end{align*}

where 
\begin{align*}
    G_{q,R}=\int_{-\infty}^{\infty}s d \Phi^{q}(\frac{s}{R\sigma_{\xxi}}),
\end{align*}
and $\Phi(\cdot)$ is the cumulative density function of a standard Gaussian distribution.
\end{theorem}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figs/integral.pdf}
    \caption{$G_{q, R}$ with different $q$, when $R\sigma_{\xxi} = 1$}
    \label{fig:integral}
\end{figure}

\paragraph{Remark}

Notice that, as Figure \ref{fig:integral} shows, $G_{q, R}$ is (near) constant that only slowly increase with $q$. In comparison, under the same setting, as shown in \citep{yin2019rademacher}, the $\epsilon-\ell_{\infty}$ adversarial training
can hurt the generalization with $\Rn[\tF]=\Theta\left(\Rn[\F]+\epsilon R\sqrt{\frac{d}{n}}\right)$, that is scale with $d$.

With the Ledoux-Talagrand Lemma and the standard generalization result with Rademachar complexity, we simply have the following corollary.

\begin{corollary}[Gap between Losses]
\label{cor:gap}
Let $\mathcal{D}$ denote the population data distribution, and define
\begin{align*}
    \Delta_{q}(\th):= \E_{\mathcal{D}}\E_{\xxi_{[q]}}\max_{\xxi_{i},i\in[q]}\ell(f_{\th}(\x+\xxi_{i}),y)-\E_{\mathcal{D}}\ell(f_{\th}(\x),y).
\end{align*}
Then for any $\delta>0$, with probability $1-\delta$, we have 
\begin{align*}
    \E_{\mathcal{D}}\ell(f_{\hat{\th}}(\x),y)& \le\E_{\mathcal{D}_{n}}\E_{\xxi_{[q]}}\max_{\xxi_{i},i\in[q]}\ell(f_{\hat{\th}}(\x+\xxi_{i}),y) - \Delta_{q}(\hat{\th})\\
    & +2L_{\varphi}\Rn[\F]+\frac{L_{\phi}G_{q,R}}{\sqrt{n}}+\sqrt{\frac{\ln(1/\delta)}{n}}.
\end{align*}


\end{corollary}

\paragraph{Remark}
Notice that, ERM has the following generalization bound:
\begin{align*}
    \E_{\mathcal{D}}\ell(f_{\hat{\th}}(\x),y)\le\E_{\mathcal{D}_{n}}\ell(f_{\hat{\th}}(\x),y)+2L_{\varphi}\Rn[\F]+\sqrt{\frac{\ln(1/\delta)}{n}}.
\end{align*}
Thus, if $\hat{\th}$ satisfies the following inequality: 
\begin{align*}
    \E_{\mathcal{D}_{n}}\E_{\xxi_{[q]}}\max_{\xxi_{i},i\in[q]}\ell(f_{\hat{\th}}(\x+\xxi_{i}),y)&-\E_{\mathcal{D}_{n}}\ell(f_{\hat{\th}}(\x),y)\\
&\le\Delta_{q}(\hat{\th})-\frac{L_{\varphi}G_{q,R}}{\sqrt{n}},
\end{align*}
which is related to the sample of $\mathcal{D}_n$, then we have a sharper generalization bound than ERM, which means we improve the generalization with the weak adversarial training.

Define
\begin{align*}
    \Delta_{q, n}(\th):=\E_{\mathcal{D_n}}\E_{\xxi_{[q]}}\max_{\xxi_{i},i\in[q]}\ell(f_{\th}(\x+\xxi_{i}),y)-\E_{\mathcal{D}}\ell(f_{\th}(\x),y),
\end{align*}
we can see that:
\begin{align*}
    \mathbb{E}_{\mathcal{D}_n\sim \mathcal{D}} \Delta_{q, n} = \Delta_{q}.
\end{align*}
{\color{red} This is not true since parameter depends on data}

And obviously, $\Delta_{q,n}$ is sub-Gaussian distributed as the loss is bounded. With the standard concentration inequality, we have constant (though small) probability that the $\x$ satisfies the desired property.

\paragraph{Remark}
Another methods is that, we can show the two estimator have different behavior in practice. For example, on the linear separable data, probably with this kinds of method we can have larger margin than ERM, but other data augmentation can also work. {\color{red} TODO}

Intuitively, the inequality means that $\hat{\th}$ is hard to attack with this kinds of weak adversarial perturbation on training set compared with the test set.
Here we introduce a more concrete example to show the condition can be satisfied in practice. Suppose that $\x| y\sim\mathcal{N}(\th^{*}y,\sigma^{2} I)$ and $y\sim\text{Unif}\{-1,1\}$. {\color{red} This is a special case of the halfspace learning, where the data are generated from the Gaussian mixture.} We use $\varphi(s)=\max(-s, 0)$.

% \begin{proposition}
% \label{prop:half_space}
% Given the model $f_{\th}$, we have that
% \begin{align*}
% % \E_{\mathcal{D}}\E_{\xxi_{[q]}}\max_{\xxi_{i},i\in[q]}\ell(f_{\th}(\x+\xxi_{i}),y)-\E_{\mathcal{D}}\ell(f_{\th}(\x),y)
% \Delta_q(\th)=G_{q,\left\Vert \th\right\Vert}.
% \end{align*}
% \end{proposition}

% \paragraph{Remark} Notice that, for $\varphi(s) = -s$, $L_{\varphi} = 1$, thus $\Delta_q(\th) - \frac{L_{\varphi} G_{q, R}}{\sqrt{n}} = (1-\frac{1}{\sqrt{n}}) G_{q, R}$ if we constrain $\|\th\| \leq R$. On the other hand, if $\|\th^*\|$ is sufficient large and $\sigma_{\xi}$ is relatively small compared with $\sigma$, then the generated data is separable with high probability. 
% In this case, the training error of standard ERM (corresponding to the term $\mathbb{E}_{\mathcal{D}_n} \ell(f_{\th}(x), y)$) and the weak adversarial training (corresponding to the term $\E_{\mathcal{D}_{n}}\E_{\xxi_{[q]}}\max_{\xxi_{i},i\in[q]}\ell(f_{\th}(\x+\xxi_{i}),y)$) are both zero. Thus, MaxUp can improve the generalization in this case.

\begin{theorem}
\label{thm:cdf}
\begin{align*}
 & \frac{1}{n}\sum_{i=1}^{n}\mathbb{E}_{\xxi_{[q]}}\min_{\xxi_{j},j\in[q]}\mathbb{I}\left\{ \th^{\top}(\x_{i}+\xxi_{j})y_{i}\le0\right\} \\
= & 1-\frac{1}{n}\sum_{i=1}^{n}\Phi^{q}\left(\frac{-\th^{\top}\x_{i}y_{i}}{\left\Vert \th\right\Vert \sigma_{\xxi}}\right),
\end{align*}
where $\Phi$ is the cdf of standard gaussian distribution.
\end{theorem}



\subsection{Linear Multi-Class Classification}

We continue to study the multi-class linear classifier. In $K$-class
classification problems, we choose $\mathcal{Y}=\{0,1\}^{\otimes K}$.
The prediction function $f_{\th}(\x):\mathbb{R}^{d}\to\mathbb{R}^{K}$,
in which, the $k$-th coordinate of $f_{\th}(\x)$ is the score that
$f_{\th}$ gives to the $k$-th class. We make prediction by choosing
the class with the highest score. Given the label $\y=[y_{1},...,y_{K}]\in\R^{K}$,
in which $y_{k}=1$ and $y_{i}=0$ for all $i\ne k$, if $\y$ belongs
to the $k$-th class. Suppose our linear classifier is defined by
\[
f_{\th}(\x)=\th^{\top}\x,\ \th=[\th_{1},...,\th_{k}]\in\R^{d\times K}.
\]
And we define 
\[
\F=\F=\{f_{\th}:\left\Vert \th\right\Vert _{2,\infty}\le R\}.
\]
And the loss is defined as $\ell(f_{\th}(\x),\y)=\varphi(\y^{\top}f_{\th}(\x))$
for some $\varphi:\mathbb{R}\to[0,B]$ that is monotonically nonincreasing
and $L_{\varphi}$-Lipschitz.

\paragraph{Theorem 4 (Extension to multi-class case)}

\[
\Rn[\ell_{\tF}]\le L_{\phi}\Rn[\ell_{\F}]+\frac{L_{\phi}G_{q,R}}{2\sqrt{n}}.
\]


\subsection{Toy Examples verifies the Theory}

Denote 
\begin{align*}
\text{Train\_Gap}_{q} & =\E_{\mathcal{D}_{n}}\E_{\xxi_{[q]}}\max_{\xxi_{i},i\in[q]}\ell(\x+\xxi_{i},y;f_{\hat{\th}})-\E_{\mathcal{D}_{n}}\ell(\x+\xxi_{i},y;f_{\hat{\th}})+\frac{L_{\phi}G_{q,R}}{\sqrt{n}},\\
\text{Test\_Gap}_{q} & =\E_{\mathcal{D}}\E_{\xxi_{[q]}}\max_{\xxi_{i},i\in[q]}\ell(\x+\xxi_{i},y;f_{\th})-\E_{\mathcal{D}}\ell(\x+\xxi_{i},y;f_{\th}).
\end{align*}
By our theory, if we have $\text{Train\_Gap}_{q}<\text{Test\_Gap}_{q}$,
then the proposed surrogate loss improves the generalization. To show
this, we conduct a simpler linear classifier toy example using Hingeloss.
Figure (\ref{fig:Train_Gap-vs-Test_Gap.}) gives the quantity of $\text{Train\_Gap}_{q}$
and $\text{Test\_Gap}_{q}$ for $q=[1,2,3,4,5]$. As shown by the
result, we indeed have $\text{Train\_Gap}_{q}<\text{Test\_Gap}_{q}$
which verifies our theory.

\begin{figure}
\begin{centering}
\includegraphics[scale=0.6]{figs/gap.pdf}
\par\end{centering}
\caption{Train\_Gap vs Test\_Gap. \label{fig:Train_Gap-vs-Test_Gap.}}
\end{figure}



==> tex/regularization.tex <==
\subsection{Maxup as a Smoothness Regularization}
%In this section, we show that, 
We provide a theoretical interpretation of 
Maxup %can be viewed 
as introducing a  smoothness regularization. 
We consider the special case of  
Gaussian data augmentation, that is, 
$\mathbb{P}(\cdot|\x) = \normal(\x, \sigma^2 \boldsymbol I)$, where $\sigma^2$ denotes a small variance parameter, and $\boldsymbol I$ the identity matrix.  
%$\mathbb{P}(\cdot|\x)$ is a Gaussian 
%Assume we use the Gaussian data augmentation, i.e. $\mathbb{P}(\cdot|\x) = \x + \xi, \xi\sim\mathcal{N}(0, \sigma^2_{\xi} I)$. 

\red{[Write in a more formal way?]}

For notation, denote by $L(\x, \theta) = \ell(f_\theta(\x), y)$ the loss at point $\x$, 
and 
\begin{align} \label{equ:Lpm}
\tilde L^{[m]}_\P(\x, \th) := \E_{\{\x_i' \}\sim \P(\cdot ~|~\x)^m} \left [ \max_{i\in [m]}
\ell(f_\th(\x_i'), y)
\right]. 
\end{align}
the expected Maxup loss at $\x$, with $m$ augmentation. 


\begin{theorem}
Let $\mathbb{P}(\cdot|\x) = \normal(\x, \sigma^2 \boldsymbol I)$ and $\tilde L^{[m]}_\P(\x, \theta)$ be defined in \eqref{equ:Lpm}. 
Assume $L(\x, \theta)$ is continuously differentiable w.r.t. $\x$. 
There exists a constant $c\in (0, \sqrt{2}]$ such that %we have 
$$
\tilde L^{[m]}_\P(\x, \th) = L(\x, \th) + 
c\sigma\sqrt{\log m} ~ \left \| \nabla_{\x} L(\x,  \th) \right\|_2 + O(\sigma^2).
$$
%(write the actual value?) 
\end{theorem}

This shows that the Maxup loss can be viewed as introducing a local Lipschitz regularization $\| \nabla_{\x} L(\x,  \th) \|_2$, which encourages the smoothness of $L(\x, \th)$ w.r.t. the input $\x$. 

\paragraph{Remark}
Some work are based on direct gradient 
norm based regularization (\url{https://openreview.net/forum?id=BkeoqIywz}) Our advantage is lower computational cost, requiring no additional backpropagation. 

Theoretical issues of gradient regularizations are discussed in \url{https://arxiv.org/pdf/1808.09540.pdf}, and connection to adversarial robustness are drawn. 

\begin{proof} 
Using Taylor expansion, we have  (need clean up, write the technical condition for bounding the residual (bounded hessian))
\begin{align*}
    & \mathbb{E}_{\x_i^\prime \sim \mathbb{P}(\cdot|\x)} \max_{i\in [q]} \ell (f_{\th}(\x_i^\prime), y)\\
    = &  \ell(f_{\th}(\x), y) + \mathbb{E}_{\x_i^\prime \sim \mathbb{P}(\cdot|\x)} \max_{i\in [q]} \left[\ell (f_{\th}(\x_i^\prime), y) - \ell(f_{\th}(\x), y)\right]\\
    = & \ell(f_{\th}(\x), y) + \sigma_{\xi} \mathbb{E}_{z_i\sim \mathcal{N}(0, I)} \max_{i\in[q]}\langle \nabla_x \ell(f_{\th}(\x), y), z\rangle \\
    & + \mathcal{O}(\sigma_{\xi}^2),
\end{align*}
where the first term $\ell(f_{\th}(x), y)$ is the empirical risk on clean data, the second term can be viewed as the smooth regularization, due to the  Lemma~\ref{lem:maxGauss} (move the Lemma to appendix?). 
\end{proof}


%With Taylor expansion, the Maxup risk on $\x$ can be written in the following alternative view:

\begin{lemma}\label{lem:maxGauss}
Let $\boldsymbol g$  be a fixed vector in $\R^d$,
and $\{\vv z_i\}$ are i.i.d. random variables from $\normal(0, \sigma^2 \vv I)$. We have 
%$\exists c\in (0, \sqrt{2}]$, $\forall x, q$, we have the following equation:
\begin{align*}
    \mathbb{E} \left [ \max_{i\in[q]}\langle \vv g, \vv z_i\rangle \right ] 
    = c_{m, \sigma} \| \vv g \|_2, 
\end{align*}
where $c_{m, \sigma}= \int XXXX$ (write the explicit formula). 
\end{lemma}
\begin{proof}
As $z_i\sim \mathcal{N}(0, I)$, the term $\langle \nabla_x \ell(f_{\th}(\x), y), z_i\rangle$ is a 1-dimensional Gaussian random variable with variance $\|\nabla_x \ell(f_{\th}(x), y)\|^2$. With the expectation of the maximum of Gaussian samples {\color{red} TODO: cite}, we have the desired result.
\end{proof}
%Notice that, $\|\nabla_x \ell(f_{\th}(\x), y)\|_2$ is the local Lipschitz constant at $\x$, and thus, Maxup is in fact minimizing the local Lipschitz constant while minimizing the empirical risk.

%\paragraph{Remark} 

==> tex/related.tex <==
\section{Related Works}
We review related literatures, including 
%We first introduce 
online hard example mining (OHEM),
%then go through the literature of 
data augmentation, 
%and finally, overview the progress in the theosy and practice of
adversarial training.



\textbf{Data Augmentation}\space\space
Recently, 
a range of regularization methods have been proposed to enhance the generalization of large deep neural networks.
Among them, MixUp~\citep[e.g.,][]{zhang2018mixup} and its variants are widely used~\citep{he2019bag}.
\red{Many of these?}
These methods force the neural networks to have local linear behaviour.
% 
Some people have tried to ensemble different kinds of data augmentations
and \red{make the networks have better performance}.
\red{~\citet{cubuk2018autoaugment} defines a search space of data augmentation and search the best policy to combine them.
~\citet{cubuk2019randaugment} makes random policy to combine different augmentation. }
~\citet{zhang2019adversarial} proposes adversarial AutoAugment, which finds a policy to maximize the training loss.
This method shares a similar intuition as \emph{MaxUp}.
However, it needs hundreds of GPU hours to search for the policy.

\red{Except for successes in practical algorithms, 
some researchers focus on understanding why and how data augmentation can help the generalization.} 
%
\blue{As providing non-i.i.d data, 
data augmentation is different from giving more data to the classifier and is hard to analyze.} 
\citet{hernandez2018data} views data augmentation as an implicit regularization.
%
They further show that
data augmentation alone can achieve the same performance or higher as regularized models.
%
\citet{chen2019invariance} gives a theoretical analysis of data augmentation based on the invariant transformations.
%
\citet{li2019enhanced} shows CNN Gaussian Process kernels and convolutional neural tangent kernels are equivalent to full \red{translation data augmentation for deep learning.?} 
%
Although some successes have been made, it is still hard to fully understand data augmentation.
Since \emph{MaxUp} has similar attributes as PGD adversarial augmented data, 
we may start from analyzing \emph{MaxUp} and then extend it to general data augmentation.\red{what is the point?}

\textbf{Adversarial Training}\space\space
%
The original idea of adversarial training is to enhance the generalization of augmented adversarial data.
% 

In practice, many works have shown that,
under some conditions,
adversarial training can improve the generalization of clean data, such as \citep{xie2019adversarial}

\citet{xie2019adversarial} uses different batch normalization layers for adversarial and clean data. 

By using extra data,
they achieve current state-of-the-art results on ImageNet.

Virtual adversarial training~\citep{miyato2015distributional} generates adversarial augmented data for unlabelled data, 
and improve the performance on semi-supervised learning tasks.
% 
\red{repetitive with earlier}
Some researchers build an analysis of the trade-off between the robustness and the generalization of clean data, e.g. \citet{zhang2019trades}.
Some~\citep{raghunathan2019hurt} find out that it can hurt the generalization of clean data but not always.
It is not clear that under which condition,
PGD adversarial training can improve the generalization of clean data. \red{what is the points?}



% \paragraph{Other Regularization Techniques}%Fighting Overfitting in Deep Learning} 
% A host of techniques have been developed to alleviate overfitting in deep learning.  
% %To alleviate this issue, several different techniques have been proposed, 
% For example, adapting different kinds of regularization to constrain the complexity of neural networks~\citep[e.g.][]{ghiasi2018dropblock, srivastava2014dropout}, and augmenting the training set with different kinds of transformation on the training data~\citep[e.g.][]{yun2019cutmix, cubuk2018autoaugment, zhang2018mixup, devries2017cutout}.
% Most of these heuristic techniques can improve the performance by a large margin but are proposed for only one or two tasks, e.g. image classification.

==> tex/remove_later.tex <==
\section{Error analysis}
We want to discuss the impact of the perturbation measure and the number of sample, by decomposing the gap between training error (with surrogate loss) and testing error (of the original loss). 
\subsection{Notation}
Assume $f\in\mathcal{F}$, where $\mathcal{F}$ is the model class. $\ell$ denotes the loss function and the goal of the natural training algorithm is minimizing the empirical risk:
\begin{align*}
    \hat{R} = \mathbb{E}_{(x_i, y_i)\sim \mathcal{D}_n} \ell(f(x_i), y_i)
\end{align*}
where $\mathcal{D}_n$ is the empirical measure of data we use.

In our algorithm, we want to minimize the following surrogate loss based on $\ell$ ({\color{red} maybe called as empirical max risk}):
\begin{align*}
    \hat{R}^\prime = \mathbb{E}_{(x_i, y_i)\sim \mathcal{D}_n} \max_{k\in [q]} \ell(f(\xi_k), y_i)
\end{align*}
where $\xi_k \sim \mathbb{P}(\cdot |x_i)$, and $\mathbb{P}(\cdot |x_i)$ is some probability mass we used to sample data based on $x_i$.

So we want to measure the gap between 
\begin{align*}
    R = \mathbb{E}_{(x, y)\sim \mathcal{D}} \ell(f(x_i), y_i)
\end{align*}
and $\hat{R}^\prime$. To do this, we introduce an additional term
\begin{align*}
    R^\prime = \mathbb{E}_{(x, y)\sim \mathcal{D}} \max_{k\in [q]} \ell(f(\xi_k), y_i)
\end{align*}
And bound the two following two terms
\begin{align*}
    G_1 = & R^\prime - \hat{R}^\prime, \\
    G_2 = & R^\prime - R,
\end{align*}
separately. The first term can be viewed as a generalization error, and the second term is a fixed error term that does not depend on the data we use.

We assume the loss is bounded, e.g. in the interval $[0, B]$. Notice that, $\ell (f(\xi_k), y_i)$ is a random variable depends on $f$ and $\mathbb{P}(\cdot|x_i)$, we need to assume some basic property of this random variable (e.g. expectation, concentration).

\begin{assumption}
Given some function class $\mathcal{F}$ and $\mathbb{P}(\cdot |x)$, for all $(x_i, y_i)\sim \mathcal{D}$ and $f\in\mathcal{F}$, we have an uniform upper bound of the tail probability of loss, i.e. $\mathbb{P}(\ell(f(\xi_k), y_i) \geq t)\leq \sigma(t)$, where $\xi_k\sim \mathbb{P}(\cdot|x_i)$.
\end{assumption}

Obviously, we can have a trivial upper bound $\sigma(t) = 1$. However, to make our analysis more meaningful, we assume $\sigma(t)$ is monotonically decreasing with $t$, with $\sigma(0)=1$, $\sigma(B)=0$. [{\color{red}, Notice that as the support of loss is bounded, it's always sub-Gaussian. However, currently it's not clear how to use this property and if it is necessary.}]
